What kinds of strong star--black-hole encounters in AGN disks occur, and how often?

Disks surrounding active galactic nuclei contain many stars and black holes, which will inevitably encounter one another. The outcome of these encounters depends on how closely and how rapidly the bodies meet. Extending previous studies, we account for initial relative velocities seeded by stochastic effects in the disk; incorporate a strong-encounter cross-section accounting for single- and binary-mediated interactions computed via direct two-body (Hill) or three-body (isolated) interactions; and present a repeated-encounter model accounting both for energy loss due to stellar encounters as well as the SMBH tidal field. We convolve our encounter model with a parametric family of natal stellar and binary populations, focused on varying binary fraction and period distribution. In our fiducial disk model, even though single-single interactions supply most encounters, binary-mediated interactions supply 68% of collisions; most encounters are well-approximated as parabolic; and stochastically-driven relative velocities are comparatively substantial and driven by gravitational perturbations from disk fluctuations and neighboring bodies. Our tools are ready to use in downstream applications, including several easily-expressed semianalytic approximations to key interaction phenomena.

==> Makefile <==
LATEX ?= pdflatex
DOCS = dynamics dynamics_supplemental
.PHONY: all clean
all:
	@for doc in $(DOCS); do \
	  for pass in 1 2 3; do \
	    $(LATEX) -interaction=nonstopmode -halt-on-error $$doc.tex > $$doc-build.txt 2>&1 || { cat $$doc-build.txt; exit 1; }; \
	  done; \
	done
clean:
	rm -f *.aux *.log *.out *.blg *.toc *Notes.bib *-build.txt $(addsuffix .pdf,$(DOCS))

